A Self-supervised Motion Representation for Portrait Video Generation

Recent advancements in portrait video generation have been noteworthy. However, existing methods rely heavily on human priors and pre-trained generative models, Motion representations based on human priors may introduce unrealistic motion, while methods relying on pre-trained generative models often suffer from inefficient inference. To address these challenges, we propose Semantic Latent Motion (SeMo), a compact and expressive motion representation. Leveraging this representation, our approach achieve both high-quality visual results and efficient inference. SeMo follows an effective three-step framework: Abstraction, Reasoning, and Generation. First, in the Abstraction step, we use a carefully designed Masked Motion Encoder, which leverages a self-supervised learning paradigm to compress the subject's motion state into a compact and abstract latent motion (1D token). Second, in the Reasoning step, we efficiently generate motion sequences based on the driving audio signal. Finally, in the Generation step, the motion dynamics serve as conditional information to guide the motion decoder in synthesizing realistic transitions from reference frame to target video. Thanks to the compact and expressive nature of Semantic Latent Motion, our method achieves efficient motion representation and high-quality video generation. User studies demonstrate that our approach surpasses state-of-the-art models with an 81% win rate in realism. Extensive experiments further highlight its strong compression capability, reconstruction quality, and generative potential.

==> sections/5_discussion.tex <==
\section{Discussion and Limitation}
\label{Discussion}

% \begin{figure}[t]\centering
% \includegraphics[width=1.0\linewidth]{img/mask_discussion.pdf}
% \vspace{-6mm}
% \caption{Motion encoding in SeMo requires minimal information, achieving good results even when 90\% of the data is masked.}
% \vspace{-1mm}
% \label{fig:mask_discussion}
% \end{figure}
% \vspace{-1mm}

% \begin{figure}[t]\centering
% \vspace{-2mm}
% \includegraphics[width=1.0\linewidth]{img/general_discussion.pdf}
% \vspace{-4mm}
% \noindent \caption{SeMo can be adapted to general video scenes.}
% \label{fig:general_discussion}
% \vspace{-8mm}
% \end{figure}
% \vspace{-1mm}

\vspace{-1mm}
\textbf{Motion encoding requires minimal information.} As demonstrated in the MAE \cite{mae2022}, model needs very minimal to generate meaningful visual content. However, in the context of motion encoding, even less information is required. The core difference between motion encoding and image encoding lies in the fact that motion encoding has a reference image. This makes much of the detailed information in the target image unnecessary. Previous methods did not make good use of the information in the reference image. In the example \cref{fig:mask_discussion}, we observe that even 90\% of the image is masked, the original video can still be reconstructed.


\noindent \textbf{Transfer to General Scenarios.} We investigated whether Motion AutoEncoder is applicable to general videos. In \cref{fig:general_discussion}, We found that in single-subject motion scenarios, Motion AutoEncoder performs well in reconstruction, even effectively learning hand movements. However, in complex multi-subject motion scenarios, noticeable distortions occur. We reproduced IMF and train them on WebVid.


\noindent \textbf{Abstract Resoning and Detail Generation.} Current video generation models, like Sora, perform temporal reasoning and pixel generation simultaneously, neglecting redundancy in motion representation. Consider how humans think – we don’t fully visualize the next state, but rather abstract conceptual representations for efficient reasoning. Video generation models could adopt similar principles: by constructing a more compact informational space through abstraction, we enable efficient inference. Subsequently, the abstract information guides the generative model in pixel synthesis, making prediction more efficient and manageable.
% Current mainstream video generation models, such as Sora-like systems, synchronously perform temporal reasoning and pixel generation. This modeling approach fails to consider the redundancy in motion representation. Consider how humans think - we don't fully visualize the next state, but rather abstract conceptual representations for reasoning in abstract spaces. Video generation models could adopt similar principles: by constructing a more compact informational space through abstraction, we enable efficient inference within this space. Subsequently, the abstract information guides the generative model in pixel synthesis, making the entire prediction process more efficient and manageable.



\noindent \textbf{Limitation.}
We found that the generated results have blurry teeth, and high-frequency areas like beards tend to flicker. We believe this is caused by the factor that: we resize data to 256x256 and compression into the latent space via SD VAE, there was significant information loss. However, our method is scalable, and we can easily extend it to higher resolutions, by maintaining the current approach.

\vspace{-2mm}



==> table/generation_facevid.tex <==
\begin{table}[t]
\centering
\caption{Audio-driven video generation comparison of various methods on the DH-FaceVid-1K dataset.}
\vspace{-2mm}
\label{tab:a2v_facevid}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{DH-FaceVid-1K}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
AniPortrait~\cite{aniportrait2024}    & 44.807       & 484.861          & 0.168          & 19.103          & 0.671           \\
Hallo2~\cite{cui2024hallo2}           & 61.803       & 698.668          & 0.155          & 20.016          & 0.658   \\
SadTalker~\cite{sadtalker2023}        & 85.447       & 610.627          & 0.328          & 14.382          & 0.538   \\
Anitalker~\cite{anitalker2024}        & 56.322       & 556.607          & 0.289          & 15.064          & 0.572    \\
Echomimic~\cite{echomimic2024}        & 69.296       & 691.534          & 0.327          & 14.218          & 0.527      \\
SeMo (Ours)                           & \textbf{27.667}       & \textbf{206.523}         & \textbf{0.095}          & \textbf{22.954}          & \textbf{0.768}     \\ \bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/generation_hdtf.tex <==
\begin{table}[t]
\centering
\caption{Audio-driven video generation comparison of various methods on the HDTF dataset.}
\vspace{-2mm}
\label{tab:a2v_hdtf}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c}{\textbf{HDTF}}                                                \\ \cline{2-8} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{Sync-C$\uparrow$} & \textbf{Sync-D$\downarrow$} \\ \hline
AniPortrait~\cite{aniportrait2024}    & 33.139       & 422.644          & 0.138          & 20.042          & 0.672          & 5.817       & 10.881     \\
Hallo2~\cite{cui2024hallo2}           & 27.447       & 276.564          & \textbf{0.105}  & 21.692          & 0.713          & \textbf{6.284}       & \textbf{8.499}     \\
SadTalker~\cite{sadtalker2023}        & 93.744       & 548.635          & 0.225          & 14.493          & 0.437          & 5.439       & 9.940     \\
Anitalker~\cite{anitalker2024}        & 41.034       & 430.082          & 0.208          & 17.434          & 0.588          & 5.927       & 8.724     \\
Echomimic~\cite{echomimic2024}        & 70.768       & 591.313          & 0.311          & 14.920          & 0.452          & 6.030       & 10.462     \\
SeMo (Ours)                           & \textbf{26.860}       & \textbf{218.414}          & 0.111          & \textbf{21.985}          & \textbf{0.739}          & 6.147       & 8.574     \\ \bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> table/model_capacity.tex <==
\begin{table}[t]
\centering
\caption{Model Capacity of various methods.}
\label{tab:capacity}
\vspace{-3mm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\makecell{Method}    & \makecell{Unsupervised} & \makecell{Long-term\\ Modeling} & \makecell{Real-time\\ Generation} & \makecell{Generic Generation\\ Pipeline} \\ \midrule
Aniportrait~\cite{aniportrait2024}  & \scalebox{1.7}{$\times$}  & \scalebox{1.7}{$\times$}  & \scalebox{1.7}{$\times$}  & \scalebox{1.7}{$\times$}     \\ 
Hallo2~\cite{cui2024hallo2}  & \scalebox{1.7}{$\times$}    & \scalebox{1.7}{$\times$}   & \scalebox{1.7}{$\times$}     & \scalebox{1.7}{$\times$}  \\ 
SadTalker~\cite{sadtalker2023}   & \scalebox{1.7}{$\times$}   & \scalebox{1.7}{\checkmark}    & \scalebox{1.7}{\checkmark}  & \scalebox{1.7}{$\times$}  \\ 
Anitalker~\cite{anitalker2024}  & \scalebox{1.7}{\checkmark}   & \scalebox{1.7}{\checkmark}    & \scalebox{1.7}{\checkmark}    & \scalebox{1.7}{$\times$}  \\ 
Echomimic~\cite{echomimic2024}  & \scalebox{1.7}{$\times$}   & \scalebox{1.7}{$\times$}    & \scalebox{1.7}{$\times$}   & \scalebox{1.7}{$\times$}    \\
SeMo~(Ours)  & \scalebox{1.7}{\checkmark}    & \scalebox{1.7}{\checkmark}     & \scalebox{1.7}{\checkmark}  & \scalebox{1.7}{\checkmark} \\

\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> table/token.tex <==
% --------------------------- Dimenshion size ---------------
\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s channel dimension on the HDTF dataset.}

\label{tab:ablation_dimension}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token}} & \multicolumn{5}{c}{\textbf{HDTF}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D32    & 29.877      & 237.652          & 0.068          & 26.916          & 0.824           \\
T1D64           & 26.174       & 214.236          & 0.066          & 27.520          & 0.835   \\
T1D128        & 24.467       & 192.702          & 0.053          & 27.587          & 0.837   \\
T1D256      & 22.629       & 157.235          & 0.048          & 28.430          & 0.865    \\
T1D512        & 21.431       & 136.738          & 0.043          & 29.12          & 0.871      \\
T1D768        & 21.424       & 135.678          & 0.042          & 29.385          & 0.872      \\
T1D1024        & \textbf{21.369}       & \textbf{133.547}         & \textbf{0.039}          & \textbf{29.430}          & \textbf{0.877}\\

\hdashline

T2D256      & 21.082       & 133.529          & 0.041          & 29.561          & 0.873      \\
T4D128      & 20.561       & 130.061          & 0.040          & 29.992          & 0.880      \\
T8D64       & \textbf{20.138}   & \textbf{128.390}    & \textbf{0.038}    & \textbf{30.180}      & \textbf{0.883} \\ \bottomrule
\end{tabular}
}

\end{table}


% ------------------------------- Token num --------------------------

\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s token length on the HDTF dataset.}
\vspace{-1mm}
\label{tab:ablation_token_length}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token Number}} & \multicolumn{5}{c}{\textbf{HDTF}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D512      & 21.431       & 136.738          & 0.043          & 29.120          & 0.871    \\
T2D256      & 21.082       & 133.529          & 0.041          & 29.561          & 0.873      \\
T4D128      & 20.561       & 130.061          & 0.040          & 29.992          & 0.880      \\
T8D64       & \textbf{20.138}   & \textbf{128.390}    & \textbf{0.038}    & \textbf{30.180}      & \textbf{0.883}     \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\end{table}






% --------------------------- Dimenshion size ---------------
\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s channel dimension on the DH-FaceVid-1K dataset.}
% \vspace{-2mm}
\label{tab:ablation_dimension1}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token Dimension}} & \multicolumn{5}{c}{\textbf{DH-FaceVid-1K}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D32    & 27.123      & 133.5          & 0.0413          & 30.38                        & 0.888           \\
T1D64           & 25.739       & 125.313          & 0.0384          & 30.948             & 0.896   \\
T1D128        & 25.414       & 121.835          & 0.038          & 31.274                & 0.898   \\
T1D256      & 24.336       & 116.858        & 0.0372        & 32.099                     & 0.899    \\
T1D512        & 23.745     & 112.166         & 0.036        & 32.132                     & 0.904      \\
T1D768        & 22.982       & 106.574         & 0.0353          & 32.696                & 0.905     \\
T1D1024        & \textbf{22.768}   & \textbf{104.768} & \textbf{0.0347}          & \textbf{32.769}          & \textbf{0.906}     \\ \bottomrule
\end{tabular}
}
% \vspace{-5mm}
\end{table}


% --------------------------- Dimenshion size -------------------------------
\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s channel dimension on the Mead dataset.}
% \vspace{-2mm}
\label{tab:ablation_dimension2}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token Dimension}} & \multicolumn{5}{c}{\textbf{Mead}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D32    & 28.344      & 97.140                    & 0.028                & 33.969            & 0.943            \\
T1D64           & 26.774        & 86.522           & 0.023                & 35.174            & 0.947    \\
T1D128        & 25.782        & 82.214             & 0.021                & 35.598            & 0.947   \\
T1D256      & 24.286        & 78.737               & 0.020                & 36.009            & 0.948     \\
T1D512        & 23.546      & 70.975                & 0.019                & 36.233           & 0.949        \\
T1D768        & 22.848        & 68.493             & 0.019                & \textbf{36.563}         & 0.953    \\
T1D1024   & \textbf{22.768}   & \textbf{67.911 }   & \textbf{0.018}       & 36.537          & \textbf{0.958 }     \\ \bottomrule
\end{tabular}
}
% \vspace{-5mm}
\end{table}


% --------------------------- Dimenshion token -------------------------------
\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s token number on the DH-FaceVid-1K dataset.}
% \vspace{-2mm}
\label{tab:ablation_tokennumber1}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token Number}} & \multicolumn{5}{c}{\textbf{DH-FaceVid-1K}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D512    & 23.745      & 112.166             & 0.036         & 32.132          & 0.904            \\
T2D256     & 23.385        & 110.907          & 0.035         & 32.691           & 0.912    \\
T4D128     & 22.961        & 110.003          & 0.033         & 32.922           & 0.919   \\
T8D64      & \textbf{22.648 }       & \textbf{108.324}          & \textbf{0.032 }        & \textbf{33.163}        & \textbf{0.922}     \\
\bottomrule
\end{tabular}
}
% \vspace{-5mm}
\end{table}


% --------------------------- Dimenshion token -------------------------------
\begin{table}[t]
\centering
\caption{Ablation studies of the latent Motion’s token number on the Mead dataset.}
% \vspace{-2mm}
\label{tab:ablation_tokennumber2}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Token Number}} & \multicolumn{5}{c}{\textbf{Mead}}                                                \\ \cline{2-6} 
& \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} \\ \hline
T1D512     & 23.546        & 70.975        & 0.019        & 36.233       & 0.949            \\
T2D256     & 23.397        & 70.372        & 0.017        & 36.991           & 0.951    \\
T4D128     & 22.925        & 69.580        & 0.016        & 37.291           & 0.956   \\
T8D64      & \textbf{22.435}        & \textbf{68.574}        & \textbf{0.014}       & \textbf{38.140}        & \textbf{0.957}     \\
\bottomrule
\end{tabular}
}
% \vspace{-5mm}
\end{table}
